TimeChat-Online: 80% Visual Tokens are Naturally Redundant in Streaming Videos

The rapid growth of online video platforms, particularly live streaming services, has created an urgent need for real-time video understanding systems. These systems must process continuous video streams and respond to user queries instantaneously, presenting unique challenges for current Video Large Language Models (VideoLLMs). While existing VideoLLMs excel at processing complete videos, they face significant limitations in streaming scenarios due to their inability to handle dense, redundant frames efficiently. We introduce TimeChat-Online, a novel online VideoLLM that revolutionizes real-time video interaction. At its core lies our innovative Differential Token Drop (DTD) module, which addresses the fundamental challenge of visual redundancy in streaming videos. Drawing inspiration from human visual perception's Change Blindness phenomenon, DTD preserves meaningful temporal changes while filtering out static, redundant content between frames. Remarkably, our experiments demonstrate that DTD achieves an 82.8% reduction in video tokens while maintaining 98% performance on StreamingBench, revealing that over 80% of visual content in streaming videos is naturally redundant without requiring language guidance. To enable seamless real-time interaction, we present TimeChat-Online-139K, a comprehensive streaming video dataset featuring diverse interaction patterns including backward-tracing, current-perception, and future-responding scenarios. TimeChat-Online's unique Proactive Response capability, naturally achieved through continuous monitoring of video scene transitions via DTD, sets it apart from conventional approaches. Our extensive evaluation demonstrates TimeChat-Online's superior performance on streaming benchmarks (StreamingBench and OvOBench) and maintaining competitive results on long-form video tasks such as Video-MME and MLVU.

==> tables/abla_drop.tex <==
\begin{table}[t]
    \small
    \centering
    \caption{Ablation study of different token dropping strategies on StreamingBench \textit{(Real-Time Visual Understanding)}. For fair comparison, all methods are evaluated with Qwen2.5VL-7B (Vanilla) without supervised fine-tuning (SFT). $\Delta$ represents accuracy retention rate (\%) relative to the full token setting.}
    \label{tab:abla_drop}
    \begin{adjustbox}{max width=0.7\columnwidth}
    \begin{tabular}{l@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}}
    \toprule
    \multirow{2}{*}{\textbf{Method w/o SFT}} & \textbf{StreamingBench} & \\
    & \textbf{(3s$\sim$24min)} & $\Delta$ \\
    \midrule
    \multicolumn{3}{c}{\textbf{Vanilla, Avg \underline{22K} Video Tokens per Video (1 fps)}} \\
    \midrule
    Qwen2.5VL-7B  & 73.7 & 100\% \\
    \midrule
    \multicolumn{3}{c}{\textbf{Drop 44.1\%, Avg \underline{12K} Video Tokens per Video}} \\
    \midrule
    \quad + VisionZip~\textsubscript{\textcolor{grey}{[CVPR 2025]}} & 72.3 & 98.1\% \\
    \quad + Pixel-level drop & 72.8 & 98.8\% \\
    \quad + Feature-level drop (frame-aware) & 73.0 & 99.1\% \\
    \rowcolor{gray!20} \quad + Feature-level drop (video-aware) & \textbf{73.4} & \textbf{99.6\%} \\
    \midrule
    \multicolumn{3}{c}{\textbf{Drop 82.5\%, Avg \underline{4K} Tokens per Video}} \\
    \midrule
    \quad + VisionZip~\textsubscript{\textcolor{grey}{[CVPR 2025]}} & 68.8 & 93.4\% \\
    \quad + Pixel-level drop & 68.8 & 93.4\% \\
    \quad + Feature-level drop (frame-aware) & \textbf{72.0} & \textbf{97.7\%} \\
    \rowcolor{gray!20} \quad + Feature-level drop (video-aware) & \textbf{72.0} & \textbf{97.7\%} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}


==> tables/offlinevideo.tex <==
\begin{table*}[t]
    \small
    \centering
    \caption{\small Results on offline long video benchmarks. We report the accuracy on the MLVU multiple-choice questions, and VideoMME without subtitles. $\dagger$ indicates the reproduced results.}
    \label{tab:long_video_benchmarks}
    % \begin{adjustbox}{max width=0.7\linewidth}
    \begin{adjustbox}{max width=1.2\columnwidth}
    \begin{tabular}{lc|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Frames}} & \multirow{2}{*}{\textbf{MLVU}} & \multirow{2}{*}{\textbf{LongVideoBench}} & \multicolumn{2}{c}{\textbf{VideoMME}} \\
    \cmidrule(lr){5-6}
    \addlinespace[1pt]
    & & & & overall & long \\
    \midrule
    \textbf{Video Length} & - & 3$\sim$120 min & 8 sec$\sim$60 min & 1$\sim$60 min & 30$\sim$60 min \\
    \midrule
    \multicolumn{6}{c}{\textbf{Open-Source Offline \videollms}} \\
    \midrule
    % Video-LLaVA-7B & 8 & 38.4 & 47.3 & - & - \\
    %Chat-UniVi-7B & 64 & - & - & - & 40.6 & 35.8 \\
    LLaMA-VID-7B & 1fps & 33.2 & - & - & - \\
    % TimeChat-7B & 96 & 30.9 & - & 30.2 & 26.1 \\
    MovieChat-7B & 2048 & 25.8 & - & 38.2 & 33.4 \\
    % Video-LLaMA2-7B & 16 & 51.7 & 48.5 & 40.6 & 35.8 \\
    LLaVA-Next-Video-7B & 32 & - & 43.5 & 46.6 & - \\
    % ShareGPT4Video-8B & 16 & - & 46.4 & 51.4 & - \\
    VideoChat2-7B & 16 & 47.9 & 39.3 & 39.5 & 33.2 \\
    LongVA-7B & 128 & 56.3 & - & 52.6 & 46.2 \\
    Kangaroo-7B & 64 & 61.0 & 54.2 & 56.0 & 46.6 \\
    Video-CCAM-14B & 96 & 63.1 & - & 53.2 & 46.7 \\
    VideoXL-7B & 128 & 64.9 & - & 55.5 & 49.2 \\
    Qwen2.5-VL-7B$\dagger$ & 1fps (100\%) & 66.9 & 61.5 & 63.2 & 50.4 \\
    \rowcolor{gray!20} Qwen2.5-VL-7B~$_{\text{w/ \module}}$ & 1fps ($\downarrow$46.2\%) & 68.6 & 61.6 & 63.4 & 51.9 \\
    \rowcolor{gray!40} Qwen2.5-VL-7B~$_{\text{w/ \module}}$ & 1fps ($\downarrow$84.6\%) & 68.8 & 59.3 & 64.9 & 56.1 \\
    \midrule
    \multicolumn{6}{c}{\textbf{Open-source Online  \videollms}} \\
    \midrule
    Dispider-7B~\textsubscript{\textcolor{grey}{[CVPR 2025]}} & 1fps & 61.7 & - & 57.2 & - \\
    VideoChat-Online-8B~\textsubscript{\textcolor{grey}{[CVPR 2025]}} & 2fps & - & - & 52.8 & 44.9 \\ \midrule
    \textbf{\model-7B} & 1fps (100\%) & 62.6 & 55.4 & 62.4 & 48.4  \\ 
    \rowcolor{gray!20} \textbf{\model-7B} & 1fps ($\downarrow$46.3\%) & 62.9 & \text{57.1} & \textbf{63.3} & \textbf{52.4} \\
    \rowcolor{gray!40} \textbf{\model-7B} & 1fps ($\downarrow$85.0\%) & \textbf{65.4} & \textbf{57.7} & 62.5 & 49.2 \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\end{table*}

==> tables/offlinevideo_old.tex <==
\begin{table*}[t]
    \small
    \centering
    \caption{Results on offline long video benchmarks. We report the accuracy on the MLVU multiple-choice questions, and VideoMME without subtitles. $\dagger$ indicates the reproduced results.}
    \label{tab:long_video_benchmarks}
    \begin{adjustbox}{max width=0.99\linewidth}
    \begin{tabular}{l@{\hspace{6pt}}l@{\hspace{8pt}}|c@{\hspace{8pt}}c@{\hspace{8pt}}c c}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Frames}} & \multirow{2}{*}{\textbf{MLVU}} & \multirow{2}{*}{\textbf{LongVideoBench}} & \multicolumn{2}{c}{\textbf{VideoMME}} \\
    \cmidrule(lr){5-6}
    \addlinespace[1pt]
    & & & & overall & long \\
    \midrule
    \textbf{Video Length} & - & 3$\sim$120 min & 8 sec$\sim$60 min & 1$\sim$60 min & 30$\sim$60 min \\
    \midrule
    \multicolumn{7}{c}{\textbf{Open-Source Offline Video MLLMs}} \\
    \midrule
    % Video-LLaVA-7B & 8 & 38.4 & 47.3 & - & - \\
    %Chat-UniVi-7B & 64 & - & - & - & 40.6 & 35.8 \\
    LLaMA-VID-7B & 1fps & 33.2 & - & - & - \\
    TimeChat-7B & 96 & 30.9 & - & 30.2 & 26.1 \\
    MovieChat-7B & 2048 & 25.8 & - & 38.2 & 33.4 \\
    % Video-LLaMA2-7B & 16 & 51.7 & 48.5 & 40.6 & 35.8 \\
    LLaVA-Next-Video-7B & 32 & - & 43.5 & 46.6 & - \\
    % ShareGPT4Video-8B & 16 & - & 46.4 & 51.4 & - \\
    VideoChat2-7B & 16 & 47.9 & 39.3 & 39.5 & 33.2 \\
    LongVA-7B & 128 & 56.3 & - & 52.6 & 46.2 \\
    Kangaroo-7B & 64 & 61.0 & 54.2 & 56.0 & 46.6 \\
    Video-CCAM-14B & 96 & 63.1 & - & 53.2 & 46.7 \\
    VideoXL-7B & 128 & 64.9 & - & 55.5 & 49.2 \\
    Qwen2.5-VL-7B$\dagger$ & 1fps & ? & 56.6 & 63.2 & 50.4 \\
    \midrule
    \multicolumn{7}{c}{\textbf{Online Video MLLMs}} \\
    \midrule
    Dispider-7B~\textsubscript{\textcolor{grey}{[CVPR 2025]}} & 1fps & 61.7 & - & 57.2 & - \\
    VideoChat-Online-8B~\textsubscript{\textcolor{grey}{[CVPR 2025]}} & 2fps & - & - & 52.8 & 44.9 \\
    \rowcolor{gray!40} \textbf{\model-7B (Ours)} & 1fps ($\downarrow$85\%) & \textbf{64.9} & \textbf{58.3} & \textbf{62.7} & \textbf{51.0} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}
